Bayesian minimisation of energy consumption in turbulent pipe flow via unsteady driving

Turbulence accounts for most of the energy losses associated with the pumping of fluids in pipes. Pulsatile drivings can reduce the drag and energy consumption required to supply a desired mass flux, when compared to steady driving. However, not all pulsation waveforms yield reductions. Here, we compute drag- and energy-optimal driving waveforms using direct numerical simulations and a gradient-free black-box optimisation framework. Specifically, we show that Bayesian optimisation is vastly superior to ordinary gradient-based methods in terms of computational efficiency and robustness, due to its ability to deal with noisy objective functions, as they naturally arise from the finite-time averaging of turbulent flows. We identify optimal waveforms for three Reynolds numbers and two Womersley numbers. At a Reynolds number of 8600 and a Womersley number of 10, optimal waveforms reduce total energy consumption by 22 % and drag by 37 %. These reductions are rooted in the suppression of turbulence prior to the acceleration phase, the resulting delay in turbulence onset, and the radial localization of turbulent kinetic energy and production toward the pipe centre. Our results pinpoint that the predominant, steady operation mode of pumping fluids through pipes is far from optimal.

==> myCommands.tex <==
\RequirePackage{xspace}   % to get your spacing straight

%--- special characters -------------------------------------------------------%
\DeclareRobustCommand{\increment}{\,d\!}
\DeclareRobustCommand{\imag}{\ensuremath{\dot{\imath}}\xspace}  % imaginary unit
\DeclareRobustCommand{\orderof}[1]{\ensuremath{\mathcal{O}\!\left(#1\right)}\xspace}     % magnitude
\DeclareRobustCommand{\real}{\ensuremath{\mathcal{R}}\xspace}        % real part

% statistical average delimiter
\DeclareRobustCommand{\lla}{\left\langle}
\DeclareRobustCommand{\rra}{\right\rangle}

% text subscripts
\DeclareRobustCommand{\analytical}{\text{ana}}
\DeclareRobustCommand{\bulk}{\text{b}}
\DeclareRobustCommand{\characteristic}{c\!h\!a}
\DeclareRobustCommand{\constant}{\text{const}}
\DeclareRobustCommand{\critical}{\text{krit}}
\DeclareRobustCommand{\initial}{i\!n\!i}
\DeclareRobustCommand{\numerical}{n\!u\!m}
\DeclareRobustCommand{\reference}{\text{ref}}
\DeclareRobustCommand{\tidal}{t\!i\!d}

% special variables
\DeclareRobustCommand{\ubulk}{\ensuremath{u_{\bulk}}\xspace}          % bulk velocity
\DeclareRobustCommand{\uhpc}{\ensuremath{u_{\text{c,HP}}}\xspace}     % Hagen-Poiseuille center line
\DeclareRobustCommand{\uref}{\ensuremath{u_{\reference}}\xspace}      % reference velocity
\DeclareRobustCommand{\oref}{\ensuremath{\omega_{\reference}}\xspace} % reference angular velocity
\DeclareRobustCommand{\nsym}{\ensuremath{n_{\text{sym}}}\xspace}      % n-fold symmetry
\DeclareRobustCommand{\tauw}{\ensuremath{\tau_{\text{w}}}\xspace}     % wall shear stress
\DeclareRobustCommand{\utau}{\ensuremath{u_{\tau}}\xspace}          % friction velocity

% non-dimensional numbers
\DeclareRobustCommand{\Courant}{\ensuremath{C\!o}\xspace} % Courant number
\DeclareRobustCommand{\Mach}{\ensuremath{M\!a}\xspace} % Mach number
\DeclareRobustCommand{\Nusselt}{\ensuremath{N\hspace{-0.20em}u}\xspace} % Nusselt number
\DeclareRobustCommand{\Nui}{\ensuremath{N\hspace{-0.27em}u_{i}}\xspace} % inner Nusselt number
\DeclareRobustCommand{\Nuo}{\ensuremath{N\hspace{-0.27em}u_{o}}\xspace} % outer Nusselt number
\DeclareRobustCommand{\Nuomi}{\ensuremath{N\hspace{-0.27em}u_{\omega,i}}\xspace}
\DeclareRobustCommand{\Nuomo}{\ensuremath{N\hspace{-0.27em}u_{\omega,o}}\xspace}
\DeclareRobustCommand{\NuS}{\ensuremath{N\hspace{-0.20em}u_{\hspace{-0.1em}s}}\xspace} % shear Nusselt number
\DeclareRobustCommand{\NuT}{\ensuremath{N\hspace{-0.27em}u_{T}}\xspace} % thermal Nusselt number
\DeclareRobustCommand{\Prandtl}{\ensuremath{P\hspace{-0.1em}r}\xspace}  % Prandtl number
\DeclareRobustCommand{\Rayleigh}{\ensuremath{R\hspace{-0.1em}a}\xspace} % Rayleigh number
\DeclareRobustCommand{\Reynolds}{\ensuremath{R\hspace{-0.1em}e}\xspace} % Reynolds number
\DeclareRobustCommand{\ReDelta}{\ensuremath{R\hspace{-0.1em}e_{\delta}}\xspace}
\DeclareRobustCommand{\Rei}{\ensuremath{R\hspace{-0.1em}e_{i}}\xspace} % inner Reynolds number
\DeclareRobustCommand{\Reo}{\ensuremath{R\hspace{-0.1em}e_{o}}\xspace} % outer Reynolds number
\DeclareRobustCommand{\Romega}{\ensuremath{R_{\omega}}\xspace}         % rotation number

\DeclareRobustCommand{\ROmega}{\ensuremath{R_{\Omega}}\xspace}         % rotation number
\DeclareRobustCommand{\Re}{\ensuremath{R\hspace{-0.1em}e}\xspace}% shear Reynolds number
\DeclareRobustCommand{\ReS}{\ensuremath{R\hspace{-0.1em}e}\xspace}% shear Reynolds number
\DeclareRobustCommand{\ROmegaDub}{\ensuremath{R^{\ast}_{\Omega}}\xspace}         % rotation number
\DeclareRobustCommand{\ReSDub}{\ensuremath{R\hspace{-0.1em}e^{\ast}_{S}}\xspace} % shear Reynolds number
\DeclareRobustCommand{\NuSDub}{\ensuremath{N\hspace{-0.27em}u^{\ast}_{S}}\xspace} % shear Nusselt number
\DeclareRobustCommand{\NuTDub}{\ensuremath{N\hspace{-0.27em}u^{\ast}_{T}}\xspace} % thermal Nusselt number

\DeclareRobustCommand{\ReTau}{\ensuremath{R\hspace{-0.1em}e_{\tau}}\xspace}
\DeclareRobustCommand{\Strouhal}{\ensuremath{S\!t}\xspace}   % Strouhal number
\DeclareRobustCommand{\Taylor}{\ensuremath{T\hspace{-0.3em}a}\xspace} % Taylor number
\DeclareRobustCommand{\Womersley}{\ensuremath{W\!o}\xspace}   % Womersley number

\DeclareRobustCommand{\RBC}{Rayleigh--B\'enard convection\xspace}
\DeclareRobustCommand{\TCF}{Taylor--Couette flow\xspace}

% special math functions
\DeclareRobustCommand{\Bessel}{\ensuremath{\mathcal{J}_{0}}\xspace}   % Bessel function of first kind and order zero

% vector operators
\renewcommand{\vec}{\boldsymbol}
\DeclareRobustCommand{\divergence}{\operatorname{div}}
\DeclareRobustCommand{\gradient}{\operatorname{grad}}
\RequirePackage{rotating} % provides sideways
\DeclareRobustCommand{\laplacian}{\vec{\Delta}}


% relations
\DeclareRobustCommand{\constraint}{\stackrel{!}{=}}

% some software names
\RequirePackage{xspace}
\RequirePackage{hyperref}
\DeclareRobustCommand{\code}[1]{\textbf{\texttt{\color{black}#1}}\xspace}
\DeclareRobustCommand{\hdf}{\href{https://en.wikipedia.org/wiki/Hierarchical_Data_Format}{\code{HDF5}}\xspace}
\DeclareRobustCommand{\mpi}{\href{https://en.wikipedia.org/wiki/Message_Passing_Interface}{\code{MPI}}\xspace}
\DeclareRobustCommand{\nsc}{\href{https://github.com/dfeldmann/nsCouette}{\code{nsCouette}}\xspace}
\DeclareRobustCommand{\tlab}{\href{https://github.com/turbulencia/Tlab}{\code{tLab}}\xspace}
\DeclareRobustCommand{\omp}{\href{https://en.wikipedia.org/wiki/OpenMP}{\code{OpenMP}}\xspace}
\DeclareRobustCommand{\python}{\href{https://www.python.org/}{\code{Python}}\xspace}
\DeclareRobustCommand{\spp}{\href{https://gepris.dfg.de/gepris/projekt/273183002?language=en}{\texttt{Turbulent Superstructures (SPP1881)}}\xspace}
\DeclareRobustCommand{\hlrn}{\href{https://www.hlrn.de/?lang=en}{North German Supercomputing Alliance (HLRN)}\xspace}
\DeclareRobustCommand{\pangaea}{\href{https://www.pangaea.de/}{Pangaea}\xspace}


% common abbreviations
\DeclareRobustCommand{\cf}{c.\,f.\xspace}
\DeclareRobustCommand{\eg}{e.\,g.\xspace}
\DeclareRobustCommand{\Eg}{E.\,g.\xspace}
\DeclareRobustCommand{\etc}{etc.\xspace}
\DeclareRobustCommand{\ie}{i.\,e.\xspace}
\DeclareRobustCommand{\Ie}{I.\,e.\xspace}
\DeclareRobustCommand{\wrt}{w.\,r.\,t.\xspace}

% draft stage
\DeclareRobustCommand{\mod}[1]{{\color{Vermillion}#1}} % \xspace
\DeclareRobustCommand{\ak}[1]{{\color{Vermillion}(\textbf{AK}: \textit{#1})}\xspace}
\DeclareRobustCommand{\df}[1]{{\color{Vermillion}(\textbf{DF}: \textit{#1})}\xspace}
\DeclareRobustCommand{\ma}[1]{{\color{Vermillion}(\textbf{MA}: \textit{#1})}\xspace}
\DeclareRobustCommand{\todo}[1]{{\color{Vermillion}(\textbf{To do}: \textit{#1})}\xspace}
\DeclareRobustCommand{\q}[1]{{\color{Vermillion}(\textbf{Question}: \textit{#1})}\xspace}

\DeclareRobustCommand{\Editor}{\item[{\color{Vermillion}Edit.}]\color{Grey}}
\DeclareRobustCommand{\RefereeA}{\item[{\color{Vermillion}Ref. A}]\color{Grey}}
\DeclareRobustCommand{\RefereeB}{\item[{\color{Vermillion}Ref. B}]\color{Grey}}
\DeclareRobustCommand{\Response}{\item[{\color{Blue}Resp.}]\color{Black}}

\newcommand{\bu}{\bm{u}}
\newcommand{\bff}{\bm{f}}
\newcommand{\bv}{{\bm{\eta}}}
\newcommand{\bs}{\bm{s}}
\newcommand{\Ta}{T_\mathrm{a}}
\newcommand{\Td}{T_\mathrm{d}}
\newcommand{\Tr}{T_\mathrm{r}}
\newcommand{\dt}{\ \mathrm{d}t}
\newcommand{\dd}{\ \mathrm{d}}
\newcommand{\tw}{\tau_\mathrm{w}}
\newcommand{\mtw}{\overline{\tau}_\mathrm{w}}
\newcommand{\mP}{\overline{P}}
\newcommand{\Um}{\overline{U}}
\newcommand{\Rem}{\overline{\Re}}
\newcommand{\Jst}{\J_{\tau,\mathrm{S}}}
\newcommand{\Jsp}{\J_{P,\mathrm{S}}}
\DeclareRobustCommand{\Amax}{\ensuremath{A_\mathrm{max}}\xspace}  
\DeclareRobustCommand{\J}{\ensuremath{\mathcal{J}}\xspace}  
\DeclareRobustCommand{\Js}{\ensuremath{\mathcal{J}_\mathrm{S}}\xspace}  

\DeclareRobustCommand{\Af}{\ensuremath{A_\mathrm{f}}\xspace}
\DeclareRobustCommand{\Dr}{\ensuremath{D_\mathrm{r}}\xspace}
\DeclareRobustCommand{\Ps}{\ensuremath{P_\mathrm{s}}\xspace}
\DeclareRobustCommand{\Ud}{\ensuremath{\Um_\mathrm{d}}\xspace}
\DeclareRobustCommand{\twb}{\ensuremath{\tau_\mathrm{w, qs}}\xspace}
\DeclareRobustCommand{\tw}{\ensuremath{\tau_\mathrm{w}}\xspace}
\DeclareRobustCommand{\Pb}{\ensuremath{P_\mathrm{qs}}\xspace}
\DeclareRobustCommand{\fd}{\ensuremath{\bm{\Pi}_{U}\xspace}}
\DeclareRobustCommand{\red}[1]{{\color{red}#1}}

